Spectral Model eXplainer: a chemically-grounded explainability framework for spectral-based machine learning models

Spectral-based machine learning models have been increasingly deployed in chemometrics and spectroscopy, where predictive accuracy is as important as explainability. Current employed eXplainable Artificial Intelligence (XAI) methods are largely adapted from tabular or generic multivariate domains, assigning relevance to isolated spectral variables rather than to the chemically meaningful spectral zones. Widely adopted tools such as SHapley Additive exPlanations (SHAP), Permutation Feature Importance (PFI), and Variable Importance in Projection scores (VIP) were not designed for the physical continuity and high collinearity of spectral data, and their variable-level outputs require post-hoc aggregation to recover zone-level information. This study introduces the Spectral Model eXplainer (SMX), a post-hoc, global, model-agnostic XAI framework that explains spectral classifiers through expert-informed spectral zones. SMX summarizes each zone via PCA, defines quantile-based logical predicates, estimates predicate relevance with perturbation in stochastic subsamples, and aggregates bag-wise rankings in a directed weighted graph summarized by Local Reaching Centrality. A key component is threshold spectrum reconstruction, which back-projects predicate boundaries to the original spectral domain in natural measurement units, enabling direct visual comparison with measured spectra. The method was evaluated on eight real spectral datasets (six based on X-ray Fluorescence--XRF and two based on Gamma-ray Spectrometry) and one synthetic benchmark with known gr

==> generated/pseudocode.tex <==
% Fragment file – included via \input{pseudocode} from main.tex
% Requires: algorithm, algpseudocode, and the breakablealgorithm
% environment defined in main.tex preamble.

\begin{breakablealgorithm}
\caption{SMX: Spectral Model eXplainer}
\label{alg:smx}
\begin{algorithmic}[1]
\Require $\mathbf{X} \in \mathbb{R}^{n \times p}$ (spectral matrix), $f$ (trained model), $\{Z_m\}_{m=1}^{M}$ (spectral zones with variable boundaries), $\mathcal{Q} = \{q_1, \ldots, q_K\}$ (quantile levels), $N_P$ (number of predicates), $B$ (number of bags), $n_b$ (subsample size), $n_{\min}$ (minimum support threshold), $\mathcal{R}$ (set of random seeds)

\Ensure $L$ (predicates ranked by global importance)

\Statex \textbf{Phase 1 --- Zone extraction and PCA aggregation}
\For{$m = 1$ to $M$}
    \State Extract sub-matrix $\mathbf{X}_{Z_m} \in \mathbb{R}^{n \times d_m}$ from $\mathbf{X}$
    \State Center: $\tilde{\mathbf{X}}_{Z_m}$
    \State Fit PCA (1 component): obtain loading $\mathbf{w}_1^{(m)}$, scores $t_i^{(m)}$, and variance explained $\mathrm{VE}^{(m)}$
\EndFor

\Statex \textbf{Phase 2 --- Predicate generation}
\State $\mathcal{P} \leftarrow \emptyset$
\For{$m = 1$ to $M$}
    \For{$k = 1$ to $K$}
        \State Compute threshold $\tau_{m,k} = Q_{q_k}(t_1^{(m)}, \ldots, t_n^{(m)})$
        \State Create $P_{m,k}^{\le}$: $t_i^{(m)} \le \tau_{m,k}$ and $P_{m,k}^{>}$: $t_i^{(m)} > \tau_{m,k}$
        \State Add $P_{m,k}^{\le}$ and $P_{m,k}^{>}$ to $\mathcal{P}$, skipping any duplicate.
    \EndFor
\EndFor
\State Build indicator matrix $\mathbf{I} \in \{0,1\}^{n \times N_P}$: $I_{i,j} = 1$ iff sample $i$ satisfies predicate $P_j \in \mathcal{P}$

\Statex \textbf{Phase 3 --- Bagging, perturbation scoring, and graph construction}
\For{each seed $r \in \mathcal{R}$}
    \State Initialize directed weighted graph $G_r = (V, E)$, $\;V \leftarrow \mathcal{P} \cup \{\mathrm{Class}_0, \mathrm{Class}_1\}$
    \For{$b = 1$ to $B$}
        \State Draw subsample $\mathcal{S}_b \subset \{1,\ldots,n\}$ of size $n_b$ without replacement (using seed $r$)
        \For{each predicate $P_j \in \mathcal{P}$ with associated zone $Z_{m_j}$ of size $d_{m_j}$}
            \State $\mathcal{S}_b^{(j)} \leftarrow \{i \in \mathcal{S}_b : I_{i,j} = 1\}$
            \If{$|\mathcal{S}_b^{(j)}| < n_{\min}$}
                \State Discard $P_j$ from bag $b$; \textbf{continue}
            \EndIf
            \State Build perturbed $\tilde{\mathbf{x}}_i$: replace $\mathbf{x}_{i,Z_{m_j}}$ with column-wise median of $\mathbf{X}_{Z_{m_j}}$; keep all other features intact
            \State Query model: $\hat{y}_i \leftarrow f(\mathbf{x}_i)$, $\;\hat{y}_i^{\mathrm{pert}} \leftarrow f(\tilde{\mathbf{x}}_i)$ for all $i \in \mathcal{S}_b^{(j)}$
            \State Compute raw impact $\operatorname{Imp}(P_j)$ according to models' output type: mean absolute change for PLS-DA or probability shift for SVM and MLP
            \State Normalize by zone length: $\operatorname{Imp}(P_j) \leftarrow \operatorname{Imp}(P_j) \;/\; d_{m_j}$
        \EndFor
        \State Sort valid predicates by $\operatorname{Imp}$ descending: $P_1^{(b)} \succ P_2^{(b)} \succ \cdots \succ P_{L_b}^{(b)}$
        \State $c^* \leftarrow$ majority predicted class among samples in $\mathcal{S}_b^{(L_b)}$
        \For{$l = 1$ to $L_b - 1$}
            \State Add edge $(P_l^{(b)} \to P_{l+1}^{(b)})$ to $G_r$ with weight $w_l = \operatorname{Imp}(P_l^{(b)}) \times \mathrm{VE}^{(m_l)}$; accumulate weight if edge already exists
        \EndFor
        \State Add terminal edge $(P_{L_b}^{(b)} \to \mathrm{Class}_{c^*})$ with weight $w_{L_b} = \operatorname{Imp}(P_{L_b}^{(b)}) \times \mathrm{VE}^{(m_{L_b})}$
    \EndFor
    \For{each predicate node $P_j \in V$}
        \State Compute $\mathrm{LRC}_r(P_j)$
        \EndFor
\EndFor

\Statex \textbf{Phase 4 --- Importance aggregation and final ranking}
\For{each predicate $P_j \in \mathcal{P}$}
    \State $\overline{\mathrm{LRC}}(P_j) \leftarrow \dfrac{1}{|\mathcal{R}|}\displaystyle\sum_{r \in \mathcal{R}} \mathrm{LRC}_r(P_j)$
\EndFor
\State Sort $\mathcal{P}$ by $\overline{\mathrm{LRC}}$ in descending order to obtain $L$
\State \Return $L$
\end{algorithmic}
\end{breakablealgorithm}

==> generated/runtime_comparison.tex <==
\begin{table}[H]
  \centering
  \scriptsize
  \setlength{\tabcolsep}{3pt}
\caption{Runtime comparison (seconds) of SMX, PFI, and SHAP across models and datasets}
\label{tab:runtime_comparison}
\begin{tabular}{lrrrrrrrrr}
  \toprule
   & \multicolumn{3}{c}{PLS} & \multicolumn{3}{c}{SVM} & \multicolumn{3}{c}{MLP} \\
   \cmidrule(lr){2-4} \cmidrule(lr){5-7} \cmidrule(lr){8-10}
  Dataset & SMX & PFI & SHAP & SMX & PFI & SHAP & SMX & PFI & SHAP \\
  \midrule
  Bank Notes & 107.5 & 73.5 & 1692.8 & 104.1 & 98.6 & 10079.1 & 67.8 & 47.5 & 1540.1 \\
  E-Cigar & 493.4 & 2479.1 & 246.7 & 273.4 & 474.4 & 370.5 & 251.9 & 370.2 & 165.8 \\
  Forage & 143.4 & 118.1 & 552.7 & 111.4 & 63.5 & 1600.1 & 115.1 & 58.4 & 487.9 \\
  Milk & 173.3 & 77.8 & 1513.6 & 142.0 & 244.0 & 28244.7 & 90.4 & 49.7 & 1363.5 \\
  Sediments & 177.3 & 53.2 & 54.9 & 86.5 & 53.6 & 103.1 & 90.7 & 52.8 & 49.7 \\
  Soil (NaI) & 50.5 & 14.6 & 42.6 & 29.0 & 16.3 & 151.9 & 29.4 & 13.7 & 43.0 \\
  Soil (XRF) & 82.8 & 37.7 & 289.9 & 72.6 & 39.6 & 2073.3 & 59.3 & 19.1 & 281.3 \\
  Soil Types & 112.2 & 126.1 & 6631.0 & 116.1 & 54.5 & 11664.0 & 109.6 & 44.5 & 5061.2 \\
  Soil Types (NaI) & 27.8 & 15.7 & 92.7 & 23.7 & 8.2 & 121.0 & 25.3 & 8.7 & 98.2 \\
  Soybean & 193.6 & 129.9 & 305.3 & 140.6 & 68.5 & 852.2 & 101.3 & 48.2 & 151.8 \\
  Sweet Pepper & 171.8 & 175.7 & 33.6 & 109.1 & 42.9 & 44.6 & 85.5 & 43.8 & 23.9 \\
  Synthetic & 54.7 & 43.1 & 1086.5 & 56.8 & 24.2 & 2292.2 & 36.9 & 16.0 & 517.3 \\
  Tomato & 142.4 & 44.1 & 52.7 & 71.4 & 46.6 & 121.2 & 73.9 & 43.9 & 47.7 \\
  \midrule
  \textbf{Mean} & \textbf{148.5} & \textbf{260.7} & \textbf{968.9} & \textbf{102.8} & \textbf{95.0} & \textbf{4439.8} & \textbf{87.5} & \textbf{62.8} & \textbf{756.3} \\
  \bottomrule
\end{tabular}
\end{table}

